Programmable Heisenberg interactions between Floquet qubits

The fundamental trade-off between robustness and tunability is a central challenge in the pursuit of quantum simulation and fault-tolerant quantum computation. In particular, many emerging quantum architectures are designed to achieve high coherence at the expense of having fixed spectra and consequently limited types of controllable interactions. Here, by adiabatically transforming fixed-frequency superconducting circuits into modifiable Floquet qubits, we demonstrate an XXZ Heisenberg interaction with fully adjustable anisotropy. This interaction model is on one hand the basis for many-body quantum simulation of spin systems, and on the other hand the primitive for an expressive quantum gate set. To illustrate the robustness and versatility of our Floquet protocol, we tailor the Heisenberg Hamiltonian and implement two-qubit iSWAP, CZ, and SWAP gates with estimated fidelities of 99.32(3)%, 99.72(2)%, and 98.93(5)%, respectively. In addition, we implement a Heisenberg interaction between higher energy levels and employ it to construct a three-qubit CCZ gate with a fidelity of 96.18(5)%. Importantly, the protocol is applicable to various fixed-frequency high-coherence platforms, thereby unlocking a suite of essential interactions for high-performance quantum information processing. From a broader perspective, our work provides compelling avenues for future exploration of quantum electrodynamics and optimal control using the Floquet framework.

==> sections/1_intro_Long.tex <==
\vspace{1em}
\noindent\textbf{Introduction}

\noindent Residing at the heart of the second quantum revolution is the capability to coherently manipulate and probe the dynamics of individual microscopic quantum systems. The power and usefulness of the quantum machines one assembles are essentially determined by the level of control one can exert on the interactions between otherwise isolated quantum bits. Extending the performance of current quantum architectures and reaching fault-tolerant quantum computation thus requires the combination of a robust quantum hardware with an inclusive interaction toolbox. Some of the most advanced and robust solid-state quantum systems have eigen-frequencies fixed by design to suppress their noise sensitivity \cite{gyenis2021moving, siddiqi2021engineering}, so engineering an extensible transverse $\mathrm{XY}$ interaction scheme in these platforms remains an outstanding challenge. 

For example, in the domain of superconducting circuits, fixed-frequency platforms such as single-junction transmon \cite{koch2007charge,paik2011observation} and fluxonium biased at the half-integer flux quantum \cite{manucharyan2009fluxonium,nguyen2019high} generally have the best coherence times. The transverse coupling is typically implemented using flux-tunable qubits, which comes at the cost of additional decoherence channels, unavoidable design overhead, and operational complexity upon scaling up. Previous parametric gate schemes to implement transverse coupling between fixed-frequency transmons relied on a small coupling term which corresponds to slow interaction rate, and involved a tunable coupling element with inherently lower coherence which degrades the qubits' operational robustness \cite{mckay2016universal,ganzhorn2019gate}.

Meanwhile, Hamiltonian engineering via periodic driving has been demonstrated as a powerful tool that opens up new avenues for explorations and discoveries of systems with exotic properties \cite{weitenberg2021tailoring}, such as anomalous Floquet topological insulators \cite{wintersperger2020realization} and discrete time crystals \cite{zhang2017observation,mi2022time,randall2021many}. Floquet engineering has also been recently proposed as a viable approach for tuning the properties of fluxonium circuits, including synthesizing degenerate quasienergies differences to induce transverse coupling between the so-called Floquet qubits \cite{huang2021engineering}.

\begin{figure*}[t]
    \includegraphics[width=\textwidth]{figures/Fig1.pdf}
    \caption{\label{fig1}\textbf{Floquet qubit}. 
    \textbf{a,} Experimental schematic involving two single-junction transmon qubits $Q_1$ (red) and $Q_2$ (blue) coupled via a shared CPW resonator resulting in an effective static coupling constant $J$ \cite{majer2007coupling}. The qubits are readout dispersively via their respective CPW resonators which are connected to a common readout bus. Microwave pulses are applied to the transmission lines situated next to the capacitor pads for qubit control.
    \textbf{b,} Dependence of quasienergies on drive parameters. 
    \textbf{c,} Population in the excited state of $Q_1$ when subjected to a microwave pulse with drive amplitude of $100~\mathrm{MHz}$, detuning $\delta=\omega_d - \omega_{01}=-40~\mathrm{MHz}$, ramping time $\tau_r$ and duration $\tau_g$. Nonadiabaticity manifests as finite oscillations for short $\tau_r$'s.
    \textbf{d,} Dependence of $P_{|1\rangle}$ oscillation amplitude, and subsequently the adiabaticity, on the ramping time $\tau_r$ and the drive amplitude for the same drive frequency from (\textbf{c}). 
    \textbf{e,} Dependence of adiabaticity on the ramping time $\tau_r$ and DRAG coefficient for a pulse with the same drive amplitude and frequency from (\textbf{c}).}
\end{figure*}

In this work, we synthesize Floquet qubits from single-junction superconducting transmon qubits with fixed static coupling, an archetype of fixed-frequency architectures, and implement an $\mathrm{XXZ}$ Heisenberg interaction between them without added circuitry. Described by the simple Hamiltonian
\begin{equation}
    \hat{\mathcal{H}}_\mathrm{XXZ} = J_\mathrm{XY}(\hat{X}\hat{X} + \hat{Y}\hat{Y}) + J_\mathrm{ZZ}\hat{Z}\hat{Z}
    \label{eqn:xxz}
\end{equation}
for a system of two coupled spin-$\nicefrac{1}{2}$, it has recently emerged as a paradigmatic model hosting intriguing physical phenomena such as spin transport \cite{jepsen2020spin}, phantom helix states in cold atoms \cite{jepsen2022long}, and photon bound states in superconducting systems \cite{morvan2022formation}. We show that the transverse $\mathrm{XY}$ spin-exchange and the longitudinal $\mathrm{ZZ}$ spin-spin rates can be tuned independently by tailoring the quasienergies with microwave pulses, leading to a fully adjustable anisotropy $\Delta=J_\mathrm{ZZ}/J_\mathrm{XY}$. 

Interestingly, we observe that a \textit{Shortcut To Adiabaticity} (STA) technique \cite{gu2019shortcuts} known as \textit{Derivative Removal by Adiabatic Gate} (DRAG) \cite{motzoi2009simple,gambetta2011analytic} helps reduce the ramping time required for adiabatic mapping, thereby promising operational optimization by pulse shaping. To validate the interaction model, the systems are transformed back to the lab frame for conventional single-qubit controls and measurements. We calibrate and characterize two-qubit $\mathrm{iSWAP}$, $\mathrm{CZ}$, and $\mathrm{SWAP}$ gates, which play important roles in quantum approximate optimization algorithms \cite{farhi2014quantum,farhi2016quantum,kivlichan2018quantum}, error mitigation using virtual distillation \cite{balint2021exponential,huggins2021virtual}, and quantum error correction \cite{fowler2012surface,ghosh2015leakage}. 

% We observe intriguing dynamical heating and dephasing, which reminisces similar effects in cold atom systems \cite{viebahn2021suppressing}. Recently, a numerical study attributed this to mixing with charge-sensitive higher states \cite{cohen2022reminiscence}. 

In addition, we show that the Floquet-engineered interaction can be broadly applied to general qudit levels. Specifically, we explore the swapping between the qutrit states $|11\rangle \leftrightarrow |02\rangle$, and employ it to implement a three-qubit $\mathrm{CCZ}$ gate, which is locally equivalent to the Toffoli gate \cite{fedorov2011implementation}. Besides being essential in factorization algorithms \cite{shor1997polynomial,haner2016factoring,gidney2021how,gu2021fast}, it enables universal reversible classical computation \cite{toffoli1980reversible}, and may streamline progress towards hardware-efficient fault-tolerance \cite{paetznick2013universal,yoder2016universal,chao2018fault}. Our work on one hand exemplifies the operational principles of Floquet qubits and on the other hand adds important tools that enhance the capabilities of fixed-frequency solid-state quantum systems to perform analog many-body quantum simulations and gate-based quantum computations.

% Our work proves the practical importance of Floquet framework in engineering quantum interactions, adds crucial quantum gates to the toolbox of fixed-frequency transmons, provides this platform with novel primitive to perform quantum simulation, and can be readily adapted to other qubits \cite{gyenis2021moving,nguyen2022scalable} as well as architectures beyond superconducting systems.




==> sections/2_floquet_Long.tex <==
\vspace{1em}
\noindent\textbf{Synthesizing Floquet qubit}

% The crux of quantum engineering is to amend additional desired terms to the static Hamiltonian describing otherwise isolated quantum systems. Among the state-of-the-art techniques, Floquet protocols have increasingly become useful across many disciplines, giving access to new properties such as artificial gauge field, exotic states of matter such as anomalous Floquet topological insulator, and to novel concepts such as discrete time crystal (see Ref. \cite{weitenberg2021tailoring} for a review). To put it simply, they provide a path to tailor otherwise inaccessible Hamiltonian.


%Short recap on Floquet
% \noindent Broadly speaking, Floquet engineering is the technique of modifying quantum systems using periodic drives, and has been shown to provide a path to tailor otherwise inaccessible Hamiltonians. Although the systems are consequently time-dependent, Floquet theorem treats them as time-independent in terms of quasi-energies and Floquet states \cite{shirley1965solution,son2009floquet}, which can be adiabatically connected to the eigenstates of the static Hamiltonian. In superconducting qubits, Floquet framework has been investigated previously in strongly driven flux qubit \cite{deng2015observation}, and recently utilized to design and implement dynamical sweet spots in fluxonium qubits \cite{huang2021engineering,mundada2021floquet}. 

%Device
\noindent The experimental device is constructed from single-junction transmon circuits forming a ring network. Each qubit is formed by two superconducting electrodes sandwiching a thin layer of aluminum oxide, resulting in a Josephson junction with Josephson energy $E_J$ shunted by a capacitor with charging energy $E_C$. The qubits are pairwise coupled via mutual coplanar waveguide (CPW) superconducting resonators designed to provide an effective coupling $J$ \cite{majer2007coupling}. Figure~\ref{fig1}a depicts an extensible section of the device consisting of two qubits along with their readout and control components.

%General Floquet physics
When a transmon is subjected to a periodic driving field with amplitude $A(t)$ at frequency $\omega_d$, it can be described by the Hamiltonian 
\begin{equation}
\begin{split}
    \hat{\mathcal{H}}(t) &= \sqrt{8E_CE_J}\hat{a}^\dagger \hat{a} - \frac{E_C}{12}(\hat{a}^\dagger + \hat{a})^4 \\ &+ A(t)\left(\hat{a}^\dagger e^{-i\omega_dt} + \hat{a} e^{i\omega_dt} \right),
\end{split}
\end{equation}
where $\hat{a}^\dagger$ ($\hat{a}$) is the creation (annihilation) operator in the harmonic oscillator basis \cite{blais2021circuit}. It follows Floquet theory \cite{shirley1965solution,deng2016dynamics} that the  solution to the Schrödinger equation $i\hbar\partial_t|\psi\rangle = \hat{\mathcal{H}}|\psi\rangle$ can be written as
\begin{equation}
    |\psi_{F,j}\rangle = e^{-i\varepsilon_jt}|u_j(t)\rangle,
\end{equation}
where $\varepsilon_j$ are the quasienergies and $|u_j(t)\rangle = \sum_{n=-\infty}^\infty e^{in\omega_d t}|u_{j,n}\rangle$ are the Floquet modes. The transition frequencies of these modes is given as a function of the drive frequency $\omega_d$ and amplitude $A$, as illustrated in Fig.~\ref{fig1}b.
\longb{Can you give some intuitive formula here?} The dynamics can be further extended for multiple pulses following multi-mode Floquet framework \cite{shirley1965solution,son2009floquet}. Therefore, the Floquet states can be modified by adjusting the amplitudes, frequencies, and relative phases of the microwave pulses (Methods).


%Adiabaticity, how we experimentally keep it adiabatic
The adiabatic mapping between the eigenstates of the transmon and the dressed states of the Floquet qubit is of central importance within Floquet framework. The general quantum state of the qubit reads $|\psi(t)\rangle = \sum_j c_j(t)|\psi_{F}(t)$, where the coefficient $c_j$ changes in time following $\dot{c}_j(t) = -\dot{A}\times \mathcal{M}(A,t)$ \cite{deng2016dynamics}, where $\mathcal{M}$ can be viewed as the dipole moment between $u_j(A,t)$ and other modes (Methods). In other words, there exists a finite transition amplitude between the Floquet modes proportional to $dA(t)/dt$, such that the one-to-one connection is only valid when the ramping time of the microwave pulse is sufficiently slow or the change of the amplitude is adequately small.

To explore the adiabatic regime's boundary, we measure the excited state population of qubit $Q_1$ after irradiating it with a cosine pulse having variable ramping time $\tau_r$ and duration $\tau_g$, at a frequency red-detuned from the $|0\rangle-|1\rangle$ transition by $40~\mathrm{MHz}$. The pulse's amplitude is fixed at $100~\mathrm{MHz}$ (in terms of on-resonant Rabi rate). Nonadiabatic effect manifests as fast oscillations in $P_{|1\rangle}$ when the pulse is changed suddenly, with shorter ramping times evidently corresponding to larger oscillation amplitudes in Fig.~\ref{fig1}c. By also varying the maximal amplitude of the pulse, we confirm that adiabaticity depends on a combination of the pulse's amplitude and ramping time (Fig.~\ref{fig1}d). Thus, longer ramping time can be used to accommodate larger drive amplitude if necessary. 

Interestingly, we find a substantial reduction in nonadiabatic effect due to pulse shaping. Fixing the maximum drive amplitude at $100~\mathrm{MHz}$, we observe that the fast oscillation amplitude can be further adjusted by adding a quadrature component to the pulse with an amplitude varying in time as $\lambda_\mathrm{DRAG}\times \dot{A}(t)$. This technique is referred to as DRAG \cite{motzoi2009simple,gambetta2011analytic}, a common STA technique \cite{gu2019shortcuts}. As shown in Fig.~\ref{fig1}e, adding a quadrature with DRAG coefficient $\lambda_\mathrm{DRAG}\approx -0.7$ to a pulse with ramping time $\tau_r=30~\mathrm{ns}$ leads to the same $P_{|1\rangle}$ as a pulse with $\tau_r=60~\mathrm{ns}$ and no DRAG. This suggests that pulse shaping and optimal control techniques should be explored within Floquet framework to further advance similar quantum operation using periodic drives.



%T1, T2
% To gauge additional detrimental effect besides nonadiabaticity, we perform coherence times measurement following standard procedure but with the application of an off-resonant pulse replacing the empty time delay. We leverage the single-shot readout capability of the experimental apparatus to pre- and post-select the results, thereby determining the population change. The data in Fig.~\ref{fig1}f shows that the echo dephasing time $T_2^E$ is reduced, while the decay time from excited to ground state $T_\downarrow$ is enhanced. We observe that this correlates with a heating effect that incoherently excites the qubit to the excited state, which has increased population at the end of the pulse application with similar exponential time constant for all amplitude values. We exclude the results corresponding to $A>85~\mathrm{MHz}$ as the onset of nonadiabatic effect appears. Despite this incoherent pumping to state $|1\rangle$, the coherence time $T_2$ is reduced by only approximately $20~\mathrm{\mu s}$, sufficient to demonstrate the protocol. A more systematic investigation of this phenomenon will be done in the future to explore potential solution to this problem.




==> sections/3_heisenberg_Long.tex <==
\vspace{1em}

\noindent\textbf{Heisenberg interaction}

\begin{figure*}[t]
    \includegraphics[width=\textwidth]{figures/Fig2.pdf}
    \caption{\label{fig2}\textbf{Floquet-engineered $\mathrm{XXZ}$ Heisenberg interaction}. \textbf{a,} Chevron pattern showing the dependence of $|01\rangle$ population on the pulses' amplitude $A_\mathrm{XY}$ and duration $\tau_g$ (upper left schematic). The qubits are first initialized in $10\rangle$. The pulses are applied at frequencies 40 MHz red(blue)-detuned from $Q_{1(2)}$'s $|0\rangle\leftrightarrow|1\rangle$ transition with DRAG coefficients $\lambda_\mathrm{DRAG}=-(+)0.6$ and ramping time $\tau_r=50~\mathrm{ns}$.
    \textbf{b,} Coherent oscillation between $|10\rangle$ and $|01\rangle$ along the optimal pulse amplitude $A_\mathrm{XY}=65.2~\mathrm{MHz}$ in (\textbf{a}). 
    \textbf{c,} Longitudinal coupling angle $\Phi_\mathrm{ZZ}$ measured after application of pulses at 40 MHz red-detuned from $Q_1$'s $|0\rangle\leftrightarrow|1\rangle$ transition (bottom left schematic). They are 200-ns-long, with ramping time $\tau_r=50~\mathrm{ns}$ and DRAG coefficient $\lambda_\mathrm{DRAG}=-0.6$. The first pulse's amplitude is fixed at $A_\mathrm{XY}=65~\mathrm{MHz}$, while the second pulse's amplitude $A_\mathrm{ZZ}$ and phase $\varphi$ are varied to tune the $\mathrm{ZZ}$ coupling rate.
    \textbf{d,} Longitudinal coupling angle $\Phi_\mathrm{ZZ}$ between the qubits after being subjected to all three pulses. $A_\mathrm{XY}$ is tuned to induce a full $|10\rangle \leftrightarrow |01\rangle$ population swap, while $A_\mathrm{ZZ}$ and $\varphi$ are varied to tune the $\mathrm{ZZ}$ rate during the swap.}
\end{figure*}

%Physics of the exchange gate. Paper by Deng and Huang.
\noindent Having established the general conditions for adiabatic mapping between undriven eigenstates and Floquet states, we next tailor the microwave pulses to engineer the $\mathrm{XXZ}$ Heisenberg interaction between the qubits as depicted in Fig.~\ref{fig1}a. It follows conventional wisdom that an $\mathrm{XY}$ exchange interaction between two coupled spins occurs when they are brought into resonance with each other. Thus, when the quasienergy differences become degenerate, a transverse coupling between the Floquet qubits occurs in the dressed frame following \cite{huang2021engineering}
    \begin{equation}
    \label{eqn:hamiltonian_xy}
        \widetilde{\mathcal{H}}_\mathrm{XY} = Jg_{1,+} g_{2,-} \hat{c}_{1,+}\hat{c}_{2,-} +\mathrm{h.c.},
    \end{equation}
where $J$ is the coupling constant, $g_{j,\mu}$ are the Fourier coefficients, and $c_{j,\mu}$ are the matrix elements in the Floquet basis associated with the qubit $Q_j$.

%Experiment to do it
Given that $Q_1$'s frequency is lower than that of $Q_2$, their quasienergy differences can be brought into resonance if $Q_1$($Q_2$) is driven with red(blue) detuned microwaves. After preparing the qubits in state $|10\rangle$, we apply two such pulses with the same duration $\tau_g$ and amplitude $A_\mathrm{XY}$ to both qubits, ensuring adiabatic condition by optimizing their ramping time $\tau_r=50~\mathrm{ns}$ and DRAG coefficient $\lambda_\mathrm{DRAG}=\mp 0.6$. We observe a population transfer to state $|01\rangle$ that forms a chevron pattern as a function of $\tau_g$ and $A_\mathrm{XY}$, signifying a transverse coupling between the qubits (Fig.~\ref{fig2}a).

Remarkably, although the interaction occurs between the Floquet qubits in the dressed frame, the adiabatic connection ascertains the exchange between the bare states after the reverse mapping, which bears resemblance to the latching mechanism in classical electronics. Indeed, at the optimal drive amplitude $A_\mathrm{XY}=65.2~\mathrm{MHz}$ (dashed line in Fig.~\ref{fig2}a), $|10\rangle$ and $|01\rangle$ exhibit coherent oscillations at a rate primarily determined by the static coupling constant $J$ (Fig.~\ref{fig2}b), consistent with the Hamiltonian given by Eq.~\ref{eqn:hamiltonian_xy}. The lack of fast oscillatory behavior as seen in Fig.~\ref{fig1}c is a clear indication of the high mapping fidelity.

%Physics of the ZZ interaction. Refer to paper by Agustin + Sizzle.
Meanwhile, the dynamical longitudinal $\mathrm{ZZ}$ coupling appears as $\tilde{\zeta}_\mathrm{ZZ}(t) = \varepsilon_{|00\rangle}(t) + \varepsilon_{|11\rangle}(t) - \varepsilon_{|10\rangle}(t) - \varepsilon_{|01\rangle}(t)$, which is in principle independent of the degeneracy required for transverse coupling. In other words, while the $\mathrm{XY}$ coupling corresponds to moving the Floquet states in opposite directions, thereby involving driving each qubit at a different frequency, the $\mathrm{ZZ}$ coupling arises from differential shifts in the qubits' quasinenergy transitions, which is most straightforwardly implemented by driving both qubits at the same frequency. Given the one-to-one mapping condition, applying microwave drives with amplitudes $A_{1,2}$ and phases $\phi_{1,2}$ to both qubits at a frequency $\omega_d$ leads to a $\mathrm{ZZ}$ rate of \cite{wei2022hamiltonian,mitchell2021hardware}
\longb{replace this equation}
\begin{equation}
    \tilde{\zeta}_\mathrm{ZZ} \approx 4\pi J\frac{A_1 A_2}{\delta_1\delta_2} \cos(\phi_1 - \phi_2).
\end{equation}

%Decribe the experiment to realize the ZZ measurement.
We proceed to induce the $\mathrm{ZZ}$ coupling between the Floquet qubits by irradiating microwave drives to both control lines at 40 MHz red-detuned from $Q_1$, with the first one having a fixed amplitude $A_\mathrm{XY}=65.2~\mathrm{MHz}$ and zero phase, while the second having parameterized amplitude $A_\mathrm{ZZ}$ and phase $\varphi$ (Fig.~\ref{fig2}, bottom left). To provide an adiabatic connection between the undriven states and the Floquet states, the pulses are sculpted to have a cosine envelope with a total duration of 200-ns. We characterize the operation by first initializing the two qubits in the superposition state $|++\rangle$, applying the pulses, perform quantum state tomography, and utilize a numerical optimization routine to extract the entangling phase $\Phi_\mathrm{ZZ}$ (Methods), which depends on the amplitude $A_\mathrm{ZZ}$ and phase $\varphi$ of the second pulse (Fig.~\ref{fig2}c).

Leveraging the fact that the transverse and longitudinal couplings depend on different pulses, we now show that both can be enabled at the same time and controlled independently. To this end, we essentially repeat the previous experiment, but having both $\mathrm{XY}$ pulses applied with fixed amplitude $A_\mathrm{XY}$ and duration $\tau_g$ that correspond to a full $|10\rangle \leftrightarrow |01\rangle$ exchange in Fig.~\ref{fig2}a,b. After integrating this swap condition into the tomographic measurement and analysis, we observe the expected dependence of $\Phi_\mathrm{ZZ}$ on the $\mathrm{ZZ}$ pulse's parameters as shown in Fig.~\ref{fig2}d, in agreement with the above description. Notably, while the transverse spin-exchange rate is primarily determined by the static coupling constant, the longitudinal spin-spin rate depends on the pulses' amplitudes and relative phase, resulting in a fully tunable anisotropy $\Delta=J_\mathrm{ZZ}/J_\mathrm{XY}$ between the qubits.



==> sections/S9_qutrit.tex <==

\noindent\textbf{$|11\rangle \leftrightarrow |02\rangle$ qutrit Haar simulation} 
\noindent
